Periodic trajectories in P-time event graphs and the non-positive circuit weight problem

P-time event graphs (P-TEGs) are specific timed discrete-event systems, in which the timing of events is constrained by intervals. An important problem is to check, for all natural numbers $d$, the existence of consistent $d$-periodic trajectories for a given P-TEG. In graph theory, the Proportional-Inverse-Constant-Non-positive Circuit weight Problem (PIC-NCP) consists in finding all the values of a parameter such that a particular parametric weighted directed graph does not contain circuits with positive weight. In a related paper, we have proposed a strongly polynomial algorithm that solves the PIC-NCP in lower worst-case complexity compared to other algorithms reported in literature. In the present paper, we show that the first problem can be formulated as an instance of the second; consequently, we prove that the same algorithm can be used to find $d$-periodic trajectories in P-TEGs. Moreover, exploiting the connection between the PIC-NCP and max-plus algebra we prove that, given a P-TEG, the existence of a consistent 1-periodic trajectory of a certain period is a necessary and sufficient condition for the existence of a consistent $d$-periodic trajectory of the same period, for any value of $d$.

==> figures/d-periodic.tex <==
\begin{tikzpicture}[node distance=.6cm and .6cm,>=stealth',bend angle=45]
\tikzset{
	myptr/.style={
		decoration={markings,mark=at position 1 with {\arrow[scale=.5]{>}}},
		postaction={decorate},
		shorten >=0.4pt}}
\tikzstyle{place}=[circle,draw=black,minimum size=3mm]
\tiny

% G(P,Q,R)
\node [place,tokens=0,label=left:{$j$}] (P1) {};
\node [place,tokens=0,label=right:{$i$},right= 4.5 cm of P1] (P2) {};
\node [place,tokens=0,label=left:{$j+n$},below= of P1] (P11) {};
\node [place,tokens=0,label=right:{$i+n$},right= 4.5 cm of P11] (P22) {};

\path (P11) -- (P22) node[midway] (cen) {};
\node [below=.5 cm of cen,anchor=center] (dots) {$\textbf{\vdots}$};
\node [left=2.25 cm of dots,anchor=east] {$\textbf{\vdots}$};
\node [right=2.25 cm of dots] {$\textbf{\vdots}$};

\node [place,tokens=0,label=left:{\tiny{$j+(d-1)n$}},below= 1cm of P11] (P111) {};
\node [place,tokens=0,label=right:{\tiny{$i+(d-1)n$}},below= 1cm of P22] (P222) {};

% Edges G(P,Q,R)
\draw (P1) edge[myptr] node[auto,swap,label={[xshift=-1.2cm]above:{$\MC_{ij}$}}] {} (P2);
\draw (P11) edge[myptr] node[auto,swap,label={[xshift=-.5cm]above:{$\MC_{ij}$}}] {} (P22);
\draw (P111) edge[myptr] node[auto,swap,label={[xshift=-1.2cm]above:{$\MC_{ij}$}}] {} (P222);
\draw (P1) edge[bend left=5,myptr] node[auto,swap,label={[xshift=0.63cm,yshift=-.15cm]above:{$\MI_{ij}$}}] {} (P22);
\draw (P11) edge[bend left=5,myptr] node[auto,swap,label={[xshift=.75cm,yshift=-.2cm]above:{$\MI_{ij}$}}] {} (dots);
\draw (dots) edge[bend left=5,myptr] node[auto,swap,label={[xshift=-.5cm,yshift=.2cm]above:{$\MI_{ij}$}}] {} (P222);
\draw (P22) edge[bend left=5,myptr] node[auto,swap,label={[xshift=-1.7cm,yshift=.4cm]below:{$\MP_{ij}$}}] {} (P1);
\draw ($(dots)-(.15,.1)$) edge[bend left=5,myptr] node[auto,swap,label={[xshift=0.5cm,yshift=-.2cm]below:{$\MP_{ij}$}}] {} (P11);
\draw (P222) edge[bend left=5,myptr] node[auto,swap,label={[xshift=-.9cm,yshift=.25cm]below:{$\MP_{ij}$}}] {} ($(dots)+(.15,-.2)$);

\draw (P2) edge[bend left=45,myptr] node[auto,swap,label={[xshift=1.5cm,yshift=.8cm]below:{$d\lambda + \MP_{ij}$}}] {} (P111);
\draw (P111) edge[bend left=45,myptr] node[auto,swap,label={[xshift=-1.3cm,yshift=-1.8cm]above:{$-d\lambda + \MI_{ij}$}}] {} (P2);

\end{tikzpicture}

